Automated Generation of Multilingual Clusters for the Evaluation of Distributed Representations

We propose a language-agnostic way of automatically generating sets of semantically similar clusters of entities along with sets of "outlier" elements, which may then be used to perform an intrinsic evaluation of word embeddings in the outlier detection task. We used our methodology to create a gold-standard dataset, which we call WikiSem500, and evaluated multiple state-of-the-art embeddings. The results show a correlation between performance on this dataset and performance on sentiment analysis.

==> data/english_corpora_comparison_avg_oov.tex <==
\begin{table}[t]
\caption{Performance comparison of GloVe vectors trained on different corpora when evaluated on their common intersection.}
\label{tbl:english-corpora-comparison}
\begin{center}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{|l|l|c|}
\hline
\multicolumn{1}{|c|}{\bf Corpus}  &\multicolumn{1}{c|}{\bf OPP}  &\multicolumn{1}{c|}{\bf Acc.}
\\ \hline
Wikipedia+Gigaword & 79.31 & 51.44 \\
Wikipedia & 77.59 & 50.21 \\
Gigaword & 75.22 & 42.15 \\
\hline
\end{tabular}
\egroup
\end{center}
\end{table}

==> data/english_results_avg_oov.tex <==
\begin{table}[t]
\caption{Performance of English word embeddings on the entire WikiSem500 dataset.}
\label{tbl:english}
\begin{center}
\bgroup
\def\arraystretch{1.5}
\begin{tabularx}{\textwidth}{|l|l|Y|Y|Y|Y|Y|}
\hline
\multicolumn{1}{|c|}{\bf Model} & \multicolumn{1}{c|}{\bf Corpus} & {\bf OPP} & {\bf Acc.} & {\bf Groups Skipped} & {\bf \% Cluster Items OOV} & {\bf \% Outliers OOV}
%\multicolumn{1}{c}{\bf Model}  &\multicolumn{1}{c}{\bf Corpus}  &\multicolumn{1}{c}{\bf OPP}  &\multicolumn{1}{c}{\bf Acc.}  
%&\multicolumn{1}{c}{\bf Groups Skipped}
%&\multicolumn{1}{c}{\bf \% Cluster Items OOV}  
%&\multicolumn{1}{c}{\bf \% Outliers OOV}
\\ \specialrule{.1em}{.1em}{.1em}
\multirow{2}{*}{GloVe} & Common Crawl          & 74.89 & 37.40 & 5  &  6.33 &  5.70 \\
                       & Wikipedia+Gigaword    & 79.85 & 50.61 & 2  &  4.25 &  4.02 \\
\hline
\multirow{4}{*}{CBOW}  & Wikipedia+Gigaword    & 84.99 & 55.80 & 2  &  4.25 &  4.02 \\
                       & Google News (phrases) & 61.42 & 21.59 & 6  & 13.68 & 15.02 \\
                       & Google News           & 62.96 & 23.02 & 6  & 13.68 & 15.02 \\
                       & Leipzig+Europarl      & 72.20 & 40.85 & 18 & 22.03 & 19.62 \\
\hline 
           Skip-Gram   & Wikipedia+Gigaword    & 84.46 & 57.66 & 2  &  4.25 &  4.02 \\
\hline
\end{tabularx}
\egroup
\end{center}
\end{table}

==> data/english_results_orig.tex <==
\begin{table}[t]
\caption{Performance of English word embeddings on entire WikiSem500 dataset.}
\label{tbl:english}
\begin{center}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{l|l|c|c|c|c|c}
\multicolumn{1}{c}{\bf Model}  &\multicolumn{1}{c}{\bf Corpus}  &\multicolumn{1}{c}{\bf OPP}  &\multicolumn{1}{c}{\bf Acc.}  
&\multicolumn{1}{c}{\parbox[b]{1.2cm}{\bf Groups\\ Skipped}}
&\multicolumn{1}{c}{\parbox[b]{1.7cm}{\bf \% Cluster\\Items OOV}}  
&\multicolumn{1}{c}{\parbox[b][][c]{1.7cm}{\centering\bf \% Outliers\\ OOV}}
\\ \hline \hline
\multirow{2}{*}{GloVe} & Common Crawl & 74.68 & 36.11 & 5 & 6.55 & 7.55 \\
              & Wikipedia+Gigaword & 81.86 & 52.75 & 3 & 7.30 & 8.70 \\
\hline
\multirow{3}{*}{CBOW} & Wikipedia+Gigaword & 83.18 & 50.13 & 2 & 4.25 & 4.02 \\
                      & Google News & 62.76 & 22.80 & 8 & 14.52 & 17.71 \\
                      & Leipzig+Europarl & 72.17 & 37.99 & 24 & 23.55 & 23.60 \\
\hline Skip-Gram & Wikipedia+Gigaword & 83.25 & 53.59 & 2 & 4.25 & 4.02
\end{tabular}
\egroup
\end{center}
\end{table}

==> data/english_vocab_sizes.tex <==
\begin{table}[t]
\caption{Vocabulary sizes of English word embeddings.}
\label{tbl:english-vocab}
\begin{center}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{|l|l|c|}
\hline
\multicolumn{1}{|c|}{\bf Model}  &\multicolumn{1}{c|}{\bf Corpus}  &\multicolumn{1}{c|}{\bf Vocabulary Size}
\\ \specialrule{.1em}{.1em}{.1em}
\multirow{2}{*}{GloVe} & Common Crawl & 2,196,017 \\
              & Wikipedia+Gigaword & 2,335,882 \\
\hline
\multirow{4}{*}{CBOW} & Wikipedia+Gigaword & 2,335,882 \\
                      & Google News (with phrases) & 3,000,000 \\
                      & Google News & $\approx$931,102 \\
                      & Leipzig+Europarl (MultiCCA) & 176,691 \\
\hline Skip-Gram & Wikipedia+Gigaword & 2,335,882 \\
\hline
\end{tabular}
\egroup
\end{center}
\end{table}

==> data/intersection_results_avg_oov.tex <==
\begin{table}[t]
\caption{Performance of English word embeddings on their common in-vocabulary intersection of the WikiSem500 dataset.}
\label{tbl:intersection}
\begin{center}
\ifICLR
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{|l|l|c|c|}
\hline
\multicolumn{1}{|c|}{\bf Model}  &\multicolumn{1}{c|}{\bf Corpus}  &\multicolumn{1}{c|}{\bf OPP}  &\multicolumn{1}{c|}{\bf Acc.}
\\ \specialrule{.1em}{.1em}{.1em}
\multirow{2}{*}{GloVe} &       Common Crawl & 76.56 & 42.78 \\
                       & Wikipedia+Gigaword & 76.19 & 47.69 \\
\hline
\multirow{4}{*}{CBOW} & Wikipedia+Gigaword          & 82.64 & 55.95 \\
                      & Google News (with phrases)  & 61.86 & 23.70 \\
                      & Google News                 & 63.98 & 25.92 \\
                      & Leipzig+Europarl (MultiCCA) & 72.57 & 41.50 \\
\hline Skip-Gram      & Wikipedia+Gigaword          & 82.08 & 56.85 \\
\hline
\end{tabular}
\egroup
\else
\bgroup
\def\arraystretch{1.5}
\begin{tabularx}{\columnwidth}{|l|l|c|c|}
\hline
\multicolumn{1}{|c|}{\bf Model}  &\multicolumn{1}{c|}{\bf Corpus}  &\multicolumn{1}{c|}{\bf OPP}  &\multicolumn{1}{c|}{\bf Acc.}
\\ \specialrule{.1em}{.1em}{.1em}
\multirow{2}{*}{GloVe} &       Common Crawl & 76.56 & 42.78 \\
                       & Wikipedia+Gigaword & 76.19 & 47.69 \\
\hline
\multirow{4}{*}{CBOW} & Wikipedia+Gigaword          & 82.64 & 55.95 \\
                      & Google News (with phrases)  & 61.86 & 23.70 \\
                      & Google News                 & 63.98 & 25.92 \\
                      & Leipzig+Europarl (MultiCCA) & 72.57 & 41.50 \\
\hline Skip-Gram      & Wikipedia+Gigaword          & 82.08 & 56.85 \\
\hline
\end{tabularx}
\egroup
\fi 
\end{center}
\end{table}

==> data/intersection_results_orig.tex <==
\begin{table}[t]
\caption{Performance of English word embeddings on their common in-vocabulary intersection of the WikiSem500 dataset.}
\label{tbl:intersection}
\begin{center}
\ifICLR
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{l|l|c|c}
\multicolumn{1}{c}{\bf Model}  &\multicolumn{1}{c}{\bf Corpus}  &\multicolumn{1}{c}{\bf OPP}  &\multicolumn{1}{c}{\bf Acc.}
\\ \hline \hline
\multirow{2}{*}{GloVe} & Common Crawl & 75.80 & 40.61 \\
              & Wikipedia+Gigaword & 78.02 & 49.42 \\
\hline
\multirow{3}{*}{CBOW} & Wikipedia+Gigaword & 79.87 & 50.38 \\
                      & Google News & 63.07 & 24.79 \\
                      & Leipzig+Europarl & 72.69 & 38.91 \\
\hline Skip-Gram & Wikipedia+Gigaword & 79.88 & 52.57
\end{tabular}
\egroup
\else
\bgroup
\def\arraystretch{1.5}
\begin{tabularx}{\columnwidth}{l|l|c|c}
\multicolumn{1}{c}{\bf Model}  &\multicolumn{1}{c}{\bf Corpus}  &\multicolumn{1}{c}{\bf OPP}  &\multicolumn{1}{c}{\bf Acc.}
\\ \hline \hline
\multirow{2}{*}{GloVe} & Common Crawl & 75.80 & 40.61 \\
              & Wikipedia+Gigaword & 78.02 & 49.42 \\
\hline
\multirow{3}{*}{CBOW} & Wikipedia+Gigaword & 79.87 & 50.38 \\
                      & Google News & 63.07 & 24.79 \\
                      & Leipzig+Europarl & 72.69 & 38.91 \\
\hline Skip-Gram & Wikipedia+Gigaword & 79.88 & 52.57
\end{tabularx}
\egroup
\fi
\end{center}
\end{table}

==> data/multilingual_results_avg_oov.tex <==
\begin{table}[t]
\caption{Performance of Non-English word embeddings on entire WikiSem500 dataset.}
\label{tbl:multilingual}
\begin{center}
\bgroup
\def\arraystretch{1.5}
\begin{tabularx}{\textwidth}{|l|Y|Y|Y|Y|Y|Y|}
\hline
\multicolumn{1}{|c|}{\bf Language} & {\bf OPP} & {\bf Acc.} & {\bf Groups Skipped} & {\bf \% Cluster Items OOV} & {\bf \% Outliers OOV} & \multicolumn{1}{c|}{\bf Vocab. Size}
%\multicolumn{1}{c}{\bf Model}  &\multicolumn{1}{c}{\bf Corpus}  &\multicolumn{1}{c}{\bf OPP}  &\multicolumn{1}{c}{\bf Acc.}  
%&\multicolumn{1}{c}{\bf Groups Skipped}
%&\multicolumn{1}{c}{\bf \% Cluster Items OOV}  
%&\multicolumn{1}{c}{\bf \% Outliers OOV}
\\ \specialrule{.1em}{.1em}{.1em}
%\multicolumn{1}{c}{\bf Language} &\multicolumn{1}{c}{\bf OPP}  &\multicolumn{1}{c}{\bf Acc.}  
%&\multicolumn{1}{c}{\parbox[b]{1.2cm}{\bf Groups\\ Skipped}}
%&\multicolumn{1}{c}{\parbox[b]{1.7cm}{\bf \% Cluster\\Items OOV}}  
%&\multicolumn{1}{c}{\parbox[b][][c]{1.7cm}{\centering\bf \% Outliers\\ OOV}}
%&\multicolumn{1}{c}{\parbox[b][][c]{1.5cm}{\centering\bf Vocab.\\Size}}
%\\ \hline \hline
Spanish & 78.44 & 48.13 & 22 & 21.55 & 17.75 & 225,950 \\
\hline German & 76.03 & 42.89 & 31 & 24.45 & 25.74 & 376,552 \\
\hline Japanese & 71.23 & 40.14 & 53 & 36.82 & 24.66 & 70,551 \\
\hline Chinese & 61.20 & 30.91 & 12 & 36.15 & 31.50 & 70,865 \\
\hline
\end{tabularx}
\egroup
\end{center}
\end{table}

==> figures/cluster_entities_orig.tex <==
\begin{figure}
    \centering
    \begin{wikidatatikz}
        \begin{scope}
            \node [class] (grandparent) {sports club};
            \node [class] (parent) [below left of=grandparent] {football club}
                edge [subclassof] (grandparent);
            \node [class] (class) [below left of=parent]  {association\\football club}
                edge [subclassof] (parent);
            \node [instance] (e2) [below of=class, xshift=-15mm]  {Manchester\\United F.C.}
                edge [instanceof] (class);
            \node [instance] (e1) [left of=e2, xshift=5mm]  {FC Barcelona}
                edge [instanceof, bend left=10] (class);
            \node [instance] (e3) [below of=class, xshift=3mm] {Real Madrid\\Club de Fútbol}
                edge [instanceof] (class);
            \node [instance] (e4) [right of=e3, xshift=-4mm] {Coritiba F.C.}
                edge [instanceof] (class);
        \end{scope}
    \end{wikidatatikz}
    \caption{Partial example of a Wikidata cluster. Arrows represent "Instance Of" relationships.}
    \label{fig:wikidata-cluster}
\end{figure}

==> figures/mst_sitelinks.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.8\textwidth]{images/mst-vs-sitelinks-fixed}
    \caption{Sitelink counts for English Wikipedia pages grouped by their associated Wikidata classes' distance to Q35120 (Entity).}
    \label{fig:mst_sitelinks}
\end{figure}

==> figures/opp_mean.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.7\textwidth]{images/opp-means}
    \caption{Outlier Position Percentage (OPP) mean scores plotted against the percentage of OOV outliers in
    a each test group.}
    \label{fig:opp_variances_r2}
\end{figure}

==> figures/opp_variance.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.7\textwidth]{images/opp-variances-r2}
    \caption{Outlier Position Percentage (OPP) scores plotted against the percentage of OOV outliers in
    a each test group.}
    \label{fig:opp_variances_r2}
\end{figure}

==> figures/outlier_class.tex <==
\begin{figure}
    \centering
    \begin{wikidatatikz}
        \begin{scope}
            \node [class] (fbclub)  {football club};
            \node [class] (soccer)  [below left of=fbclub] {association \\ football club}
                edge [subclassof] (fbclub);
            \node [class] (football) [below right of=fbclub] {American \\ football team}
                edge [subclassof] (fbclub);
            
            \node [instance] (pats) [right of=football] { New England \\ Patriots }
                edge [instanceof] (football);
        \end{scope}
    \end{wikidatatikz}
    \caption{Example of a relationship between a cluster and an $\oone$ class outlier. Dashed arrows represent "Subclass Of" relationships.}
    \label{fig:wikidata-o1}
\end{figure}

==> figures/outlier_mst_depth.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.7\textwidth]{images/mst_depth_dist}
    \caption{Distribution of Wikidata classes' distance to Q35120 (Entity).}
    \label{fig:mst_dist}
\end{figure}

==> sections/handling_oov.tex <==
\section{Sanely Handling Out-of-Vocabulary Words}

One thing not addressed by \citet{camacho2016find} is how out-of-vocabulary (OOV)
items should be handled. Because our dataset is much larger and contains a wider variety of words,
we have extended their work to include an additional scoring metric which better encapsulates the performance
of vector sets trained on different corpora.

First, recall the definition of the Outlier Position Percentage (OPP) score from \citet{camacho2016find}:
\begin{equation}
\label{eqn:orig-opp}
OPP(D) = \sum_{W\in D} \frac{\frac{OP(W)}{\lvert W\rvert - 1}}{\lvert D\rvert},
\end{equation}
where $W$ is a test case, and $OP(W)$ is the position in which the true outlier is ranked by the vectors
(the outlier is detected if it is placed at zero-indexed position $\lvert W\rvert$). Restated in terms 
of test \textit{groups}, we have the following:
\begin{equation}
\label{eqn:opp}
% TODO: Remove outer level summation
OPP(D) = \sum_{\langle C,O\rangle\in D} \frac{\sum_{o\in O}\frac{OP(C\cup\{o\})}{\lvert C\rvert}}
{\sum_{\langle C^\prime, O^\prime\rangle \in D}\lvert O^\prime\rvert}
\end{equation}

There are two approaches to handling out-of-vocabulary entities: use a sentinel vector to represent
all such entities or discard such entities entirely. The first approach is simpler, but it has a number
of drawbacks; for one, a poor choice of sentinel can have a drastic impact on results. For example, an
implementation which uses the zero vector as a sentinel and defines 
$sim(\vec{x},\vec{0})=0\,\forall \vec{x}$ places many non-out-of-vocabulary outliers at a large disadvantage
in a number of vector spaces, for we have found that negative compactness scores\footnote{See \citet{camacho2016find} for definition of compactness score.} are rare. The second approach avoids
deliberately introducing invalid data into the testing evaluation, but comparing scores across vector
embeddings with different vocabularies is difficult due to them having different in-vocabulary subsets of the
test set.

%We have developed two means of addressing the shortcomings of the latter approach, which we refer to as the
%\textit{intersecting} and \textit{extrapolating} methods.
We have opted for the latter approach, computing the results on both the entire dataset and on only the 
intersection of in-vocabulary entities between all evaluated vector embeddings. This allows us to compare
embedding performance both when faced with the same unknown data and when evaluated on the same, 
in-vocabulary data.
